Stable Model-based Control with Gaussian Process Regression for Robot Manipulators

Computed-torque control requires a very precise dynamical model of the robot for compensating the manipulator dynamics. This allows reduction of the controller's feedback gains resulting in disturbance attenuation and other advantages. Finding precise models for manipulators is often difficult with parametric approaches, e.g. in the presence of complex friction or flexible links. Therefore, we propose a novel computed-torque control law which consists of a PD feedback and a dynamic feed forward compensation part with Gaussian Processes. For this purpose, the nonparametric Gaussian Process regression infers the difference between an estimated and the true dynamics. In contrast to other approaches, we can guarantee that the tracking error is stochastically bounded. Furthermore, if the number of training points tends to infinity, the tracking error is asymptotically stable in the large. In simulation and with an experiment, we demonstrate the applicability of the proposed control law and that it outperforms classical computed-torque approaches in terms of tracking precision.

==> fig/manipulator.tex <==

\newcommand{\nvar}[2]{%
    \newlength{#1}
    \setlength{#1}{#2}
}

% Define a few constants for drawing
\nvar{\dg}{0.3cm}
\def\dw{0.25}\def\dh{0.5}
\nvar{\ddx}{1.5cm}

% Define commands for links, joints and such
\def\link{\draw [double distance=1.5mm, very thick] (0,0)--}
\def\joint{%
    \filldraw [fill=white] (0,0) circle (5pt);
    \fill[black] circle (2pt);
}
\def\grip{%
    \draw[ultra thick](0cm,\dg)--(0cm,-\dg);
    \fill (0cm, 0.5\dg)+(0cm,1.5pt) -- +(0.6\dg,0cm) -- +(0pt,-1.5pt);
    \fill (0cm, -0.5\dg)+(0cm,1.5pt) -- +(0.6\dg,0cm) -- +(0pt,-1.5pt);
}
\def\robotbase{%
    \draw[rounded corners=8pt] (-\dw,-\dh)-- (-\dw, 0) --
        (0,\dh)--(\dw,0)--(\dw,-\dh);
    \draw (-0.5,-\dh)-- (0.5,-\dh);
    \fill[pattern=north east lines] (-0.5,-1) rectangle (0.5,-\dh);
}

% Draw an angle annotation
% Input:
%   #1 Angle
%   #2 Label
% Example:
%   \angann{30}{$\theta_1$}
\newcommand{\angann}[2]{%
    \begin{scope}[red]
    \draw [dashed, red] (0,0) -- (1.2\ddx,0pt);
    \draw [->, shorten >=3.5pt] (\ddx,0pt) arc (0:#1:\ddx);
    % Unfortunately automatic node placement on an arc is not supported yet.
    % We therefore have to compute an appropriate coordinate ourselves.
    \node at (#1/2-2:\ddx+8pt) {#2};
    \end{scope}
}

% Draw line annotation
% Input:
%   #1 Line offset (optional)
%   #2 Line angle
%   #3 Line length
%   #5 Line label
% Example:
%   \lineann[1]{30}{2}{$L_1$}
\newcommand{\lineann}[4][0.5]{%
    \begin{scope}[rotate=#2, blue,inner sep=2pt]
        \draw[dashed, blue!40] (0,0) -- +(0,#1)
            node [coordinate, near end] (a) {};
        \draw[dashed, blue!40] (#3,0) -- +(0,#1)
            node [coordinate, near end] (b) {};
        \draw[|<->|] (a) -- node[fill=white] {#4} (b);
    \end{scope}
}

% Draw mass annotation
% Input:
%   #1 mass label offset (optional)
%   #2 link angle
%   #3 link length
%   #4 mass label
% Example:
%   \massann[1]{30}{2}{$m_1$}
\newcommand{\massann}[4][0.4]{%
    \begin{scope}[rotate=#2, black,inner sep=2pt]
    	\filldraw [fill=black] (#3/2,0) circle (2pt);
    	\node[] at (#3/2,#1)  {#4};
    \end{scope}
}
% Define the kinematic parameters of the three link manipulator.
\def\thetaone{120}
\def\Lone{2}
\def\thetatwo{30}
\def\Ltwo{2}

\begin{tikzpicture}
    \robotbase
    \begin{scope}[shift=(0:0), rotate=-90]
    \angann{\thetaone}{$q_1$}
    \lineann[1.2]{\thetaone}{\Lone}{$l_1$}
    \link(\thetaone:\Lone);
    \joint
    \node[] at (0,-0.5)  {$\tau_1$};
    \begin{scope}[shift=(\thetaone:\Lone), rotate=\thetaone]
        \angann{\thetatwo}{$q_2$}
        \lineann[-1.5]{\thetatwo}{\Ltwo}{$l_2$}
        \link(\thetatwo:\Ltwo);
        \joint
        \node[] at (0,-0.5)  {$\tau_2$};
        \node[] at (-0.2,0.5)  {$m_1$};
        \begin{scope}[shift=(\thetatwo:\Ltwo), rotate=\thetatwo]
                \grip
                \node[] at (0,0.7)  {$m_2$};
        \end{scope}
    \end{scope}
    \end{scope}
    \draw[->] (\Lone,0) -- node[right] {$g$} (\Lone,-\dh);
\end{tikzpicture}

